A Golden Age: Conspiracy Theories' Relationship with Misinformation Outlets, News Media, and the Wider Internet

Do we live in a "Golden Age of Conspiracy Theories?" In the last few decades, conspiracy theories have proliferated on the Internet with some having dangerous real-world consequences. A large contingent of those who participated in the January 6th attack on the US Capitol fervently believed in the QAnon conspiracy theory. In this work, we study the relationships amongst five prominent conspiracy theories (QAnon, COVID, UFO/Aliens, 9/11, and Flat-Earth) and each of their respective relationships to the news media, both authentic news and misinformation. Identifying and publishing a set of 755 different conspiracy theory websites dedicated to our five conspiracy theories, we find that each set often hyperlinks to the same external domains, with COVID and QAnon conspiracy theory websites having the largest amount of shared connections. Examining the role of news media, we further find that not only do outlets known for spreading misinformation hyperlink to our set of conspiracy theory websites more often than authentic news websites but also that this hyperlinking increased dramatically between 2018 and 2021, with the advent of QAnon and the start of COVID-19 pandemic. Using partial Granger-causality, we uncover several positive correlative relationships between the hyperlinks from misinformation websites and the popularity of conspiracy theory websites, suggesting the prominent role that misinformation news outlets play in popularizing many conspiracy theories.

==> causality.tex <==
\section{Causality}







==> conspiracy-ecoystem.tex <==
sec:conspiracy-focused-datasetsec:conspiracy-focused-dataset\section{The Internal Conspiracy Ecosystem}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/conspiracy_overlap.png}
\caption{\textbf{Conspiracy Interaction: 9/11  to COVID}--- Example of how a 9/11 conspiracy site (911forum.org.uk) links to and promotes COVID conspiracy theories.}
\label{figure:nine11-covid}
\end{figure}
We begin by first examining the interactions among conspiracy websites themselves. While researchers have found that individuals who believe one conspiracy theory are more likely to believe in another~\cite{goertzel1994belief}, the interconnections and patterns of how these websites support one another are largely unknown. In this section, we examine our five conspiracy theories' interactions, identify the important website hubs in these communities, concluding that QAnon remains a prominent outlet and repository of conspiracy theories generally, not just those specific to Q. This largely accords with reporting that QAnon has become a ``big tent conspiracy theory'' that constantly incorporates new claims and theories~\cite{Roose2021}.


\subsection{Conspiracy Interaction}
Despite seemingly being five unique conspiracy theories, QAnon, Flat-Earth, COVID, UFOs, and 9-11 conspiracy theories have significant interactions with each other. To determine how each of these websites feed into one another, we first calculated the interconnections between the 848 total conspiracy websites that we had gathered. Despite the conspiracy websites being gathered and chosen independently, each group of conspiracy theory websites has come to reference each other. 

We see in Figure~\ref{fig:conspiracy-domain-connections} that each group of conspiracy websites have at least some interaction with every other conspiracy theory group. While the levels of interaction vary, each group of websites feeds into the other groups. For a concrete example, as shown in Fig~\ref{figure:nine11-covid}, COVID conspiracies like the Plandemic are often referenced on even 9/11 conspiracy sites. QAnon especially seems to dominate in this respect, often referencing the largest set of different conspiracy theories. Flat Earth conspiracy theories appear on the opposite end of the spectrum, linking to relatively few of the other conspiracy groups. We do note that despite this that our list of Flat Earth websites does connect to 20 different QAnon websites. Overall, we do note that the domain overlap between the different conspiracy theories suggests that each conspiracy theory website group (besides QAnon) largely serves a different community.

\paragraph{QAnon dominance} As seen in Figure~\ref{fig:conspiracy-domain-connections}, QAnon websites connect to the majority of every other conspiracy theory's websites except for Flat Earth. QAnon websites connect to 71\% of the 9/11 websites, 66\% of the UFO/Aliens websites, and 53\% of COVID conspiracy websites. This largely supports reporting that QAnon has become a catch-all for those that believe in conspiracy theories generally. As reported by the New York Times, QAnon has incorporated elements of other conspiracy theories including those about the assassination of John F. Kennedy, UFOs, and 9/11~\cite{Roose2021}. This largely concurs with our empirical results. Similarly, each of these different conspiracy websites groups has significant ties to QAnon. All conspiracy groups have connections to at least 20 different QAnon websites, with the COVID conspiracy websites pointing to 58 different QAnon websites. This shows that as QAnon has grown, many of these other conspiracy communities have begun to echo and perhaps incorporate its beliefs. 

\paragraph{Flat Earth Weakness}
We note that flat earth websites have the weakest links to the other sets of conspiracy websites. Although flat earth websites have connections to each type of conspiracies, flat earth websites have the least amount of connections. We note that one possible reason could be that we collected the smallest amount of flat-earth sites, only accumulating 88 different websites. Another possible explanation is that while the other conspiracy theories presented here posit that the U.S. or some other cabal is actively keeping information away from the public, Flat Earth, in contrast, posits that that science and perhaps reason itself is somewhat flawed. This lack of political orientation could help explain the paucity of connections between Flat Earth and the other websites.  We leave full exploration of this phenomenon to future work.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/conspiracy-hubs.png} 
\caption{\textbf{Conspiracy Website Hubs}--- Top 200 hubs in the five category conspiracy network as determined by the hub centrality metric. %\todo{make half height like other graph}%\todo{Can you create a PDF image of this? Looks a little blurry otherwise}
}
\label{figure:hubs}
\vspace{-1pt}
\end{figure}

\subsection{HITS Analysis}
To understand the structure of the full conspiracy ecosystem, we build a hyperlink graph centered around these conspiracies using the {Hypertext Induced Topic Selection} ({HITS}) algorithm~\cite{Kleinberg1997}. We perform this analysis to determine which set of conspiracy theory websites are important within this ecosystem. Starting with the 848 different~conspiracy domains documented earlier as our \textit{root set} of domains, we build a \textit{base set} of domains by collecting the domains link to and that both link back to these websites. In addition, we run this analysis again taking into account all the all domains that we scraped (misinformation, authentic news, non-news, and conspiracy domains) to ascertain the relatively important news and non-news websites.. In the directed graph of domains connected to conspiracy websites, there are 330K~domains and 771K~directed edge connections. In the directed graph of domains that are connected to all domains that we consider there are 5.1M nodes and 13.0M edges.

Per {HITS}, we discern both \textit{hub} and \textit{authority} central domains~\cite{LinkAnalysis}. Hub domains are defined as domains that point to many ``high authority domains and which are themselves high-value domains''. A hub typically has a large out-degree. Authority domains are defined as ``valuable and information-dense domains'' pointed to by many other domains. An authority ordinarily has a high in-degree. Due to the nature of the authority metric, authorities tend to be globally popular domains. 
\begin{table}
\centering
\small
\begin{tabular}{lrrr}
\toprule
{Domain} & {Hub} & {Authority}  & {Category}  \\
\midrule
8kun.top              &   0.499    &   0.013   &   QAnon \\
stillnessinthestorm.com                &   0.228    &   0.0.18   &   QAnon  \\
forum.tfes.org &   0.076    &    0.0008  &   Flat Earth  \\
flatrock.org.nz                    &  0.055   &   0.0008   &   Flat Earth  \\
nowtheendbegins.com                    &  0.122    &   0.015   &   COVID  \\
childrenshealthdefense.org             &   0.090   &   0.021   &   COVID \\
alienexpanse.com                &  0.067   &   0.0005   &   UFO/Aliens \\
gralienreport.com                  &   0.067    &   0.0009   &   UFO/Aliens \\
911bloger.com   &    0.118     & 0.009   &   9/11  \\
911forum.org.uk   &   0.112    &   0.002  &   9/11  \\
\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs per Conspiracy Category}---The top two domain hubs in each conspiracy category from the network graph built from 863 different conspiracy domains as a root set.}
\vspace{-20pt}
\label{table:conspiracy-hubs}
\end{table}


\begin{table}
\centering
\small
\begin{tabular}{lrrr}
\toprule
{Domain} & {Hub} & {Authority}  & {Category}  \\
\midrule
theguardian.com            &   0.013439    &   $4.661 \times 10^{-6}$   &   Authentic News \\
nytimes.com               &   0.01221    &   $4.740 \times 10^{-6}$    &    Authentic News \\
abovetopsecret.com &   0.012121    &    $2.350 \times 10^{-6}$   &   Misinformation  \\
freerepublic.com                    &  0.01044  &   $3.382 \times 10^{-6}$    &   Misinformation  \\
skyscrapercity.com                    &  0.004559    &  $1.113 \times 10^{-6}$    &   Non News  \\
goodreads.com            &   0.004261   &   $4.225 \times 10^{-6}$    &   Non News \\
\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs in non-Conspiracy Categories}---The top two domain hubs in each conspiracy category from the network graph built from 848 different conspiracy domains as a root set. Alexa rank from January 1, 2021.}
\vspace{-20pt}
\label{table:conspiracy-hubs}
\end{table}


\begin{figure*}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/misinfo-connections.png}
\label{fig:misinfo-sub1}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/mainstream-connections.png}
  \label{fig:authentic-sub2}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/nonnews-connections.png}
  \label{fig:nonnews-sub2}
\end{subfigure}
  \caption{Interaction among the conspiracy, misinformation, authentic news, and non-news websites. Our set of misinformation websites have links to the largest percentages of websites in each conspiracy category. Conversely, non-news related websites seem to rarely reference conspiracy theories or link to their websites. Conspiracy theory websites themselves seem to reference misinformation and authentic news at approximately the same rate. For example, QAnon websites has links to 80\% of our authentic news websites and 80\% of our misinformation  websites, }
  \label{figure:conspiracies-to-different-types}
\end{figure*}

\paragraph{QAnon Hubs}
The top QAnon hubs within our conspiracy centered graph include {8kun.top} and {stillnessinthestorm.com} as seen in Table~\ref{table:conspiracy-hubs} and pictured in Fig~\ref{figure:hubs}. {8kun.top} is the home of QAnona and where the progenitor of the conspiracy theory formerly posted "drops" or cryptic messages about the conspiracy theory. {8kun.top} points to 101 of the remaining 862 conspiracy theory and connects to every category of conspiracy theory, attesting to its prominence. This further confirms QAnon's role as a home of conspiracy theories. {stillnessinthestorm.com} is a blog/news site that often posts about QAnon and how current events fit into the conspiracy theory. Others, including the Columbia Journalism Review, have already documented its role in spreading conspiracies and misinformation.

\paragraph{Other Significant Hubs}
In addition to the dominant QAnon hubs, various other popular and prominent conspiracy websites play key role key roles within this conspiracy ecosystem. The most prominent Flat Earth website in our graph is associated with the ``International Flat Earth Research Society''. The International Flat Earth Research Society was founded in 1956 by Samuel Shenton and believes that the earth is a  disc with the North Pole at its center. An ice wall, in turn, surrounds the disc, protecting those inside from space ~\cite{Picheta2019}.

One of the most important COVID hubs in our set of websites is connected to the Children's Health Defense Non-Profit group. Founded by Robert F. Kennedy Jr., this non-profit has spread large amounts of misinformation about traditional vaccines. Since the start of the COVID-19 pandemic, the website has been home to a large number of conspiracy theories surrounding COVID-19 vaccines. As documented by the Digital Forensic Research Lab~\cite{Hanley2021}, the video ``Covid Vaccine Secrets'' that advocates against COVID vaccination and initially posted by childrenshealthdefense.org, was broadcasted and reposted by 21 different misinformation websites under the new title ``If People Get Jabbed After Watching This They Are Beyond Saving.''





==> conspiracy-score.tex <==
\section{Incoherence Score}
As seen in Section~\ref{sec:polarization-conspiracy}, polarization is part of explaining a website's penchant toward extreme material, but it is not the only factor. Robertson et al~\cite{robertson2018auditing} found that some misinformation websites have seemingly no bias at all. Misinformation websites like {rt.com} and {globalresearch.ca}  appear to have little partisan bias, yet are assuredly more extreme than sites like {cnn.com} and the {dailywire.com}. In this section, we propose a new metric \textbf{\textit{Incoherence Score}}, based on political polarization data \textit{and} conspiracy-oriented linking. We again define conspiracy-oriented websites as those that have more connections to conspiracy websites than to non-news or authentic news websites. This new metric provides a new means of understanding a given website's penchant for conspiracy as well as political polarization.
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/misinformation-division.png} 
\caption{\textbf{Classification of Websites Based on Polarization and Conspiracy Proximity}--- Using a simple threshold on the polarization level of a website and the number of conspiracy domains that it links to, one can differentiate between authentic news and misinformation.
}
\label{figure:classification}
\end{figure}

As seen in Figure ~\ref{figure:classification}, using simple thresholding across polarization levels and each website's percentage of conspiracy-oriented connections, we can correctly classify the majority of misinformation and authentic news sites that are both within our dataset and that of Robertson et al~\cite{robertson2018auditing}, and that we recorded as having connections to at least 100 other domains (N= 518). Using this simple approach with just two inputs, the percentage of conspiracy-oriented connections and the website's polarization level, we achieve a 91.3\% accuracy after using a Support Vector Machine (SVM) to decide on the boundary. We  note that this approach is highly interpretable; it is fairly easy to explain why a given website was labeled as misinformation or as authentic.  

This approach achieves a 93.4\% precision and a false positive rate of 2.5\%. A drawback of this approach is several misinformation websites are falsely labeled as authentic news, with a false-negative rate of 22.1\%. These misinformation websites do not link to conspiracy materials often, evidencing a flaw in this simplified approach to classification.   simple to explain why a given website was classified   We note, however, given that this approach is fairly confident about websites it classifies correctly, we utilize parts of this boundary drawing to create our new metric \textbf{\textit{Incoherence Score}}.



Taking the drawn boundary for classification, we now define \textbf{\textit{Incoherence Score}}. To create this score, we utilize a function of the distance of each website to the boundary dividing misinformation from authentic news. This is the same as how Support Vector Machines perform classification and we utilize the Support Vector machine that drew our boundary to calculate this score. Putting this all together we define a website's \textbf{\textit{Incoherence Score}} the SVM probability value derived from a point's distance to the boundary dividing misinformation from authentic news. Derived as such, \textbf{\textit{Incoherence Score}} values vary from 0 (non-extreme) to 1 (extreme).

Looking at the scores for the different groups of sites as shown in Table~\ref{table:least-coherent}, we see that among the authentic news sites that were misclassified, nearly all were hyper-partisan websites. For several, it is questionable whether they truly are authentic news websites. For example, the most extreme mainstream site, {humanevents.com} is a known hyper-conservative site. For example, on the day of writing, the top story on the site is ``THE DUCHESS IS A VICTIM AND FOOTBALL IS GAY'' (emphasis not added). 

\begin{table}
    \small
    \centering
    \begin{tabularx}{.49\columnwidth}{Xr}
    \toprule
    Domain &  Incoherence Score  \\
    \midrule
    teaparty.org     &   ~1.0 \\
    americanjournalreview.com   &   ~1.0 \\
    
    usdefensewatch.com & ~1.0 \\
    oathkeepers.org  &   ~1.0 \\
    thecommonsenseshow.com         &   ~1.0 \\
    newstarget.com & ~1.0 \\
    healthnutnews.com & ~1.0 \\
    disclose.tv  & ~1.0 \\
    eutimes.net & ~1.0 \\
    theconservativetreehouse.com & ~1.0\\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{0.49\columnwidth}{Xr}
    \toprule
    Domain &  Incoherence Score  \\
    \midrule
    humanevents.com             &   0.951 \\
    freedomworks.org             &   0.944 \\
    kenyonreview.org       &   0.920 \\
    ronpaulinstitute.org & 0.844\\
    heritage.org & 0.791 \\
    \scriptsize{davidstockmanscontracorner.com} & 0.755 \\
    dissentmagazine.org               &   0.718 \\
    worldnewsdailyreport.com             &   0.705 \\
    consortiumnews.com & 0.694 \\
    amsterdamnews.com & 0.577 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Least Coherent Misinformation (left)  and Authentic News Websites (right)}---Based on the distance of a given website from the boundary dividing misinformation and authentic news, we devise a website's \textit{Incoherence}. As seen the most Incoherent mainstream sites are hyper-partisan websites. }
   \vspace{-10pt}
    \label{table:least-coherent}
\end{table}


==> dead.tex <==
\begin{comment}
\begin{table}
    \small
    \centering
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    QAnon &  Unique URLs  \\
    \midrule
    zerohedge.com      &   39,654 \\
    thegatewaypundit.com     &   20,038 \\
    rt.com         & 19,418 \\
   naturalnews.com   &   18,090\\
    breitbart.com             & 16,261 \\
    theepochtimes.com   &   9,527 \\
    sputniknews.com &   8,597 \\
    bitchute.com & 7,681 \\
    beforeitsnews.com & 7,604 \\
    nypost.com         &   6,911 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Covid  &  Unique URLs  \\
    \midrule
    healthimpactnews.com      &   2,909 \\
    bitchute.com     &   804 \\
    naturalnews.com   &   664\\
    zerohedge.com   &   582 \\
    \mbox{off\-guardian.org} &   486 \\
    greenmedinfo.com & 470 \\
    rt.com & 404 \\
    geoengineeringwatch.org        &   357 \\
    breitbart.com       &   311
    \\
    lifesitenews.com & 310 \\
    \bottomrule
    \end{tabularx}
    
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    9/11 &  Unique URLs  \\
    \midrule
    globalresearch.ca      &   2,419 \\
    prisonplanet.com    &   2,181 \\
    rawstory.com   &   1,323\\
    infowars.com   &   1,158 \\
    whatreallyhappened.com  &   979 \\
    veteranstoday.com & 912 \\
    \scriptsize{informationclearinghouse.info} & 891 \\
    wikileaks.org         &   796 \\
    rt.com      &   694\\
    corbettreport.com & 660 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Fla Earth  &  Unique URLs  \\
    \midrule
    breitbart.com      &   63 \\
    bitchute.com     &   57 \\
    naturalnews.com   &   37\\
    rense.com   &   35 \\
    thegatewaypundit.com &   34 \\
    rt.com & 33 \\
  nypost.com & 33 \\
    icr.org         &   30 \\
    zerohedge.com       &   18
    \\
    wnd.com & 16 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    UFO/Aliens &  Unique URLs  \\
    \midrule
    coasttocoastam.com      &   1,809 \\
    rt.com     &   509 \\
    sputniknews.com   &   453\\
    collectiveevolution.com   &   437 \\
    disclose.tv  &   401 \\
    abovetopsecret.com & 352 \\
    rense.com & 321 \\
    nypost.com        &   306 \\
    beforeitsnews.com       &   298 \\
   \mbox{ancient-code.com} & 226 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Top Misinformation News Websites linked to by Conspiracy Theory Websites Groups}---As noted conspiracy websites make high use of misinformation websites, with each group utilizing misinformation news websites to different degrees.}
   \vspace{-20pt}
    \label{table:misinfo_top_link_in}
\end{table}
\end{comment}


\begin{comment}
\begin{figure*}
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/qanon-conspiracy-connect-overlap.png}
\label{fig:qanon-sub1}
\end{subfigure}%
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/flat-conspiracy-connect-overlap.png}
  \label{fig:flat-sub2}
\end{subfigure}
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/covid-conspiracy-connect-overlap.png}
  \label{fig:covid-sub2}
\end{subfigure}
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/ufo-conspiracy-connect-overlap.png}
  \label{fig:ufo-sub2}
\end{subfigure}
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/nine11-conspiracy-connect-overlap.png}
  \label{fig:nine11-sub2}
\end{subfigure}
 \caption{\textbf{Domain overlap between conspiracy theory categories}---The different conspiracy theories direct users to largely different sets of websites. QAnon, believed to be a catch-all for many different conspiracy theories, has the highest connection overlap with the different conspiracy communities, directing users to various other conspiracy theory websites. }
\end{figure*}
\end{comment}



\begin{comment}

\end{comment}


\begin{comment}
\begin{table}
\centering
\small
\begin{tabular}{lrll}
\toprule
{Domain} & {Hub} & {Authority}  & {Category}  \\
\midrule
8kun.top              &   0.499    &   0.013   &   QAnon \\
stillnessinthestorm.com                &   0.228    &   0.018   &   QAnon  \\
forum.tfes.org &   0.076    &    0.0008  &   Flat-Earth  \\
flatrock.org.nz                    &  0.055   &   0.0008   &   Flat-Earth  \\
nowtheendbegins.com                    &  0.122    &   0.015   &   COVID  \\
childrenshealthdefense.org             &   0.090   &   0.021   &   COVID \\
alienexpanse.com                &  0.067   &   0.0005   &   UFO/Aliens \\
gralienreport.com                  &   0.067    &   0.0009   &   UFO/Aliens \\
911bloger.com   &    0.118     & 0.009   &   9/11  \\
911forum.org.uk   &   0.112    &   0.002  &   9/11  \\
\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs per Conspiracy Category}---The top two domain hubs in each conspiracy category from the network graph built from 863 different conspiracy domains as a root set.}
\vspace{-10pt}
\label{table:conspiracy-hubs}
\end{table}
\end{comment}


\begin{comment}
\begin{table}
\centering
\small
\begin{tabular}{lrrr}
\toprule
{Domain} & {Hub} & {Authority}  & {Category}  \\
\midrule
theguardian.com            &   0.013439    &   $4.661 \times 10^{-6}$   &   Authentic News \\
nytimes.com               &   0.01221    &   $4.740 \times 10^{-6}$    &    Authentic News \\
abovetopsecret.com &   0.012121    &    $2.350 \times 10^{-6}$   &   Misinformation  \\
freerepublic.com                    &  0.01044  &   $3.382 \times 10^{-6}$    &   Misinformation  \\
skyscrapercity.com                    &  0.004559    &  $1.113 \times 10^{-6}$    &   Non News  \\
goodreads.com            &   0.004261   &   $4.225 \times 10^{-6}$    &   Non News \\
\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs in non-Conspiracy Categories}---The top two domain hubs in each conspiracy category from the network graph built from 863 different conspiracy domains as a root set. Alexa rank from January 1, 2021.}
\vspace{-10pt}
\label{table:news-hubs}
\end{table}
\end{comment}


\begin{comment}
\begin{table}
\centering
%\scriptsize
\tiny
\begin{tabular}{lrrlrrlrr}
\toprule
{Authtenic News} & {Hub} & {Authority} & {Misinformation} & {Hub} & {Authority}  &{Non-News} & {Hub} & {Authority}  \\
\midrule
theguardian.com            &   0.013   &   $4.66 \times 10^{-6}$   & abovetopsecret.com &   0.012    &    $2.35 \times 10^{-6}$ & skyscrapercity.com &  0.0046   &  $1.11 \times 10^{-6}$ \\
nytimes.com               &   0.012    &   $4.74 \times 10^{-6}$     &freerepublic.com                    &  0.010  &   $3.38 \times 10^{-6}$  & goodreads.com            &   0.0043   &   $4.22 \times 10^{-6}$\\
huffingtonpost.com & 0.012  & $4.57\times 10^{-6}$ & dailykos.com &  0.0078 & $3.94 \times 10^{-6}$& pyschologytoday.com & 0.0028 & $4.42\times 10^{-7}$ \\
wired.com & 0.0073  &$4.54 \times 10^{-6}$ & commondreams.org &  0.0047&$3.69\times 10^{-6}$ & cambridge.com & 0.0028 &  $4.75\times 10^{-7}$\\
npr.org & 0.0073 &$6.80 \times 10^{-7}$ & dailycaller.com & 0.0046&$4.19\times 10^{-6}$ &
inc.com & 0.0026 & $3.93\times 10^{-6}$ \\
washingtonpost.com & 0.0066& $4.73 \times 10^{-6}$ & theepochtimes.com & 0.0045& $3.72\times 10^{-6}$ & 
espn.com & 0.0023 & $4.01\times 10^{-6}$ \\
cnn.com  & 0.0066& $4.70\times 10^{-6}$ & unz.com  & 0.0042&$2.45\times 10^{-6}$   &
scribd.com & 0.0020 & $4.49\times 10^{-6}$ \\
cnet.com & 0.0063 & $4.30\times 10^{-6}$ & amerircanthinker.com & 0.0042& $3.43\times 10^{-6}$  & aarp.com & 0.0017 & $2.05\times 10^{-7}$ \\
foxnews.com & 0.0059& $4.62\times 10^{-6}$ & nypost.com &  0.0040&  $4.64\times 10^{-6}$ &
womenshealthmag.com & 0.0016 & $2.75\times 10^{-6}$ \\
alternet.org & 0.0057& $6.36\times 10^{-6}$ & pjmedia.com & 0.0037& $3.52\times 10^{-6}$ & marriot.com & 0.0020 & $7.52\times 10^{-9}$ \\



\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs in non-Conspiracy Categories}---The top ten domain hubs in each news category from the network graph built from full news and conspiracy ecosystem as the root set .}
\vspace{-10pt}
\label{table:news-hubs}
\end{table}
\end{comment}





\begin{table}
\centering
\small
\begin{tabular}{llllll}
\toprule
{Authentic News} & {QAnon} & {COVID}  & {UFO/Aliens} & {9/11} & {Flat-Earth}  \\
\midrule
 & cultish &  ambitious & credible & unvarnished  & zetetic \\
 & virtual  &unvaccinated & out-of-this-world & insensitive & skeptic \\
 & moronic &big & vicious & unexpected   &real\\
 & loudest & israeli &  top-heavy  & mixed &idiotic\\
 & viral  &elgiible & detailed & arabian &false \\
 \toprule
{Misinformation} & {QAnon} & {COVID}  & {UFO/Aliens} & {9/11} & {Flat-Earth}  \\
\midrule
 & questionable &  separate & new & positive  & much-maligned \\
 & amazing  &broad & much-discussed & ridiculous & falsifiable \\
 & worthy &unrelated & sensational & serious  &infamous\\
 & untouched &neoconservative &  real  &typical &newest\\
 & vocal  &racial & possible & unprecedented &real \\
 
\bottomrule
\end{tabular}
\caption{\textbf{Adjectives most associated with Conspiracy Theories based on Word2Vec articles model}---The top adjectives associated with each conspiracy theory based on all scraped authentic news articles. Authentic news websites tend to be highly skeptical of conspiracy theories. Misinformation websites tend to take conspiracies at face-value. }
\vspace{-10pt}
\label{table:adjectives-associated}
\end{table}




We analyze our five conspiracy theories' websites' interactions, the important websites in each community, and finally how misinformation, authentic news, and non-news-related websites interact with our set of conspiracy theories.
%\todo{This section is too long compared to others. 14 pages versus 1--2. I'd consider whether you can split it up, at least into 2 sections.}

%\todo{This level of summarizing key results is not important up front, if anything, I would try to work it into each subsection at the end to make sure it really pops. Its confusing without appropriate context.} 
%The interconnections and patterns of how different types of conspiracy theory websites are largely unknown. Furthermore, how each of these conspiracy theories individually interacts with the news media and the wider Internet is even more opaque. 
 \begin{figure*}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/qanon-overlap3.png}
\label{fig:qanon-sub1}
\end{subfigure}%
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/nine11-overlap3.png}
  \label{fig:flat-sub2}
\end{subfigure}

\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/covid-overlap3.png}
  \label{fig:covid-sub2}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/ufo-overlap3.png}
  \label{fig:ufo-sub2}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/flat-overlap3.png}
  \label{fig:nine11-sub2}
\end{subfigure}
\caption{\textbf{Percentage of Domains Referenced From One Conspiracy Category to Another}---Websites associated with each conspiracy connect to a different percentage (number domains of a category of conspiracy theory referenced) of other conspiracies' websites. Except for connections with QAnon, most conspiracies have low inter-connectivity. Flat-Earth has the weakest set of connections with other conspiracies.}
\label{fig:conspiracy-domain-connections}
\end{figure*}

%The relatively low inter-connectivity amongst conspiracies suggests that these different conspiracy theories serve different communities. Somewhat bucking this trend, QAnon websites have the strongest connections with the other conspiracy theories.
 

\subsection{The Intra-Conspiracy Ecosystem}
How different conspiracy theory websites interact with each other is largely unknown. We therefore first look at how our sets of conspiracy theory websites are connected (how many domains of one category of conspiracy theory are referenced by another).
In addition to looking at domain overlap between conspiracy theory websites, we build a domain-centered hyperlink graph centered around these websites and apply the {HITS} algorithm~\cite{Kleinberg1997}. Starting with the 863~conspiracy theory domains documented earlier as our \textit{root set} of domains, we build a \textit{base set} of domains by collecting the domains with hyperlink connections to these websites (using all the data that we scraped and collected from CommonCrawl as described in Section~\ref{sec:dataset}). In the directed graph of domains connected to conspiracy theory websites, there are 365K~domains and 796K~directed edge connections. 
%\todo{It's not clear to me based on this description how you found all the domains that point to conspiracy sites. Is this only of the subset of sites in the four categories?}

%\todo{Just because people tend to believe more than one conspiracy doesn't necessarily mean we would expect domain overlap be large, right? I'm surprised it was ``more than initially expected''. We also say ``initially expected'' three times in this paragraph :P}
Prior research has suggested that people who believe one conspiracy theory are more likely to believe in others~\cite{goertzel1994belief}; we thus initially expected some amount of interconnection between each conspiracy theory group. We see here that despite being independently curated, every conspiracy theory group has at least some interaction with every other group (Figure~\ref{fig:conspiracy-domain-connections}). However, while there are instances of mutual references as seen in Figure~\ref{fig:conspiracy-domain-connections}, such as the COVID conspiracy ``Plandemic'' being referenced even on a 9/11 conspiracy theory website (Figure~\ref{figure:nine11-covid}), this appears to be a rarer occurrence based on the raw overlap percentages. 

%\todo{This sentence confuses me because it doesn't seem to explain domain overlap: } 
% I don't think you can make that claim. Having two websites doesn't indicate that they don't have the same audience or community. The relatively low domain overlap between the different conspiracy theories appears to suggest that each conspiracy theory website group (besides QAnon) largely serves a different community.  

%\todo{I've commented out a bunch of text that I don't think helps the story line about the connectivity between conspiracy and instead just describes 1--2~websites. I don't have a strong opinion, if you want to add it back, but I didn't think it furthers the story line, and if anything distracted me. If we do think this is important, it might be better expressed just as a table of the most important hubs for each conspiracy.}

 %\todo{Cite? What should it have been?}. 
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{figures/conspiracy_overlap.png}
\end{subfigure}
\caption{\textbf{Conspiracy Interaction: 9/11  to COVID}--- Example of how a 9/11 conspiracy theory website (\mbox{911forum.org.uk}) hyperlinks to and promotes COVID conspiracy theories.}
\label{figure:nine11-covid}
\end{figure}
%The ecosystem amongst the conspiracy theory websites is further displayed in , with relative sizes of the nodes determined by the hub centrality metric from HITS analysis. QAnon especially seems to dominate, referencing the largest set of different conspiracy theories. QAnon websites have the deepest interconnections with the other conspiracy theory groups
%\todo{Strikes me a little weird for you to say: intersection is small (in previous paragraph), but also there is intersection (this paragraph). What you can do instead is just say the numbers (rather than giving a value judgement on its size) and then dive into what intersects more with what.}
%\todo{why? Is it related to 9/11 in any way, or is it just coincidence?}
%dedicated to uncovering ``\textit{the secrets of prime number 17 (Q)}'', has connections
\paragraph{QAnon} QAnon is most connected to other conspiracies (Figure~\ref{figure:hubs}); QAnon websites connect to 20\% of 9/11 websites, 29\% of UFO/Aliens websites, 42\% of COVID websites, and 7.1\% of Flat-Earth websites. For example, the largest hub in Figure~\ref{figure:hubs}, the QAnon website {wqth.wordpress.com} connects to every conspiracy theory, except for Flat-Earth. Conversely, all conspiracy groups have connections to at least 2~QAnon websites, with COVID conspiracy theory websites linking to 25~QAnon sites. Our results support news reports that QAnon has become a catch-all for conspiracy theories. As reported by the New York Times, QAnon has incorporated elements of other conspiracy theories including those concerning John F. Kennedy's assassination, UFOs, and 9/11~\cite{Roose2021}.
% \todo{you don't actually show this --- links alone aren't enough.}
%as QAnon has grown, other conspiracy communities have begun to echo and incorporate its beliefs. 

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/included-hubs3.png} 
\caption{\textbf{Conspiracy Theory Website Hubs}--- Top 200 hubs in the five category conspiracy network as determined by the hub centrality metric. The size of the nodes are determined by the hub centrality metric calculated with HITS. We see QAnon conspiracy theory websites as the largest hubs within the conspiracy ecosystem.}
\label{figure:hubs}
%\vspace{-10pt}
\end{figure}
%appear on the opposite end of the spectrum to QAnon, linking to relatively few of the other types of conspiracies. A

%%clusters. 
%One possible reason for the paucity of interconnections between Flat-Earth and the other conspiracy groups could be that we collected a small amount of Flat-Earth sites, only accumulating 99 different websites. 
\paragraph{Flat-Earth} As seen in Figures~\ref{fig:conspiracy-domain-connections} and~\ref{figure:hubs}, Flat-Earth websites are the least connected to other conspiracies. Although Flat-Earth websites \emph{do} have connections to each other type of conspiracies, Flat-Earth websites have the least amount of connections.
For instance, the most prominent Flat-Earth website, {forum.tfes.org} (``International Flat-Earth Research Society'') has connections with only QAnon and 9/11.\footnote{The International Flat-Earth Research Society was founded in 1956 by Samuel Shenton and promotes the belief that the Earth is a flat disc with the North Pole at its center. An ice wall, in turn, surrounds the disc, protecting the people inside from space~\cite{Picheta2019}.} Despite being a relatively old conspiracy theory and having the most opportunity to influence the other conspiracy theories, we do not see much interaction between Flat-Earth websites and other conspiracy types.  

One possible explanation for this paucity of interconnections is that while the other conspiracy theories posit that the U.S. or some other cabal is keeping information from the public, Flat-Earth posits that science and perhaps reason itself are flawed~\cite{russell1991inventing}. This lack of political orientation could help explain the lack of hyperlinks from Flat-Earth to the other conspiracy theory websites~\cite{landrum2021differential}. We leave the full exploration of this to future work.

\begin{table}
\centering
\small
\begin{tabular}{llll}
\toprule
{Category} &{Domain} & {Hub} & {Authority}   \\
\midrule
Multiple/Forum & {8kun.top} & 0.681 & $1.02 \times 10^{-2}$   \\
Multiple/Forum &{theburningplatform.com}& 0.209 &$1.26 \times 10^{-2}$ \\
QAnon &wqth.wordpress.com             &   0.124 
    &   $6.70 \times 10^{-4}$
 \\
QAnon &greatawakening.win               &   0.103
    &   $4.17 \times 10^{-3}$  \\
 Flat-Earth &forum.tfes.org &   0.0598
    &    $2.56\times 10^{-3}$
    \\
 Flat-Earth &flatrock.org.nz                    & 0.0426
   &  $5.26\times 10^{-4}$
    \\
COVID &nowtheendbegins.com                    & 0.0954
   &   $1.31\times 10^{-2}$
    \\
COVID &childrenshealthdefense.org             &   0.0709
  &  $1.69 \times 10^{-2}$
     \\
UFO/Aliens  &alienexpanse.com                &  0.0527   &   $3.34\times 10^{-4}$
     \\
    UFO/Aliens & gralienreport.com                  &  0.0521 &
  $1.18\times 10^{-3}$ \\
9/11  & 911bloger.com   &    0.0883   & $7.24\times 10^{-3}$
    \\
9/11  &911forum.org.uk   &   0.0850  &   $1.35\times 10^{-3}$
     \\
\bottomrule
\end{tabular}
\caption{\textbf{Top Hubs per Conspiracy Category}---The top two domain hubs in each conspiracy theory category from the network graph built from the 766 categorized conspiracy theory websites after running HITS analysis.
}
\label{table:conspiracy-hubs}
\end{table}
\paragraph{COVID} COVID, UFOs/Aliens, and 9/11 conspiracies have a level of connectivity with other conspiracies between that of QAnon and Flat-Earth. COVID websites connect with 25~Qanon, 10~9/11, 6~UFO/Aliens, and 1~Flat-Earth website(s). One of the most important COVID hubs, belonging to the Children's Health Defense Non-Profit, {childrenshealthdefense.org} has played a significant role in the spread of COVID-19 misinformation. Founded originally under the name World Mercury Project in 2011 by Robert F. Kennedy Jr., this non-profit has spread large amounts of misinformation about traditional vaccines. Since the start of the COVID-19 pandemic, the website promoted several videos and articles containing conspiracy theories targeting COVID-19 vaccines~\cite{Hanley2021}.


%\todo{what site? is it the children's health defense or is it another site that connects to children's health defense}
 %As documented by the Digital Forensic Research Lab~\cite{Hanley2021}, the video ``Covid Vaccine Secrets'' that advocates against COVID vaccination and initially posted by childrenshealthdefense.org was broadcast and reposted by 21 different misinformation websites under the new title ``If People Get Jabbed After Watching This They Are Beyond Saving.''

\paragraph{9/11} 9/11 websites also have a middling level of interconnectivity with other conspiracies with connections to 10~QAnon, 12~COVID, 8~UFO/Aliens, and 2~Flat-Earth websites. The major 9/11 hub 911bloger.com, a site dedicated to the 911 Truth Movement, is an offshoot of another 9/11 conspiracy theory website. According to the website's About page, the website is dedicated to the mission statement on 911truth.org, namely: \textit{TO EXPOSE the official lies and cover-up surrounding the events of September 11th, 2001 in a way that inspires the people to overcome denial and understand the truth; namely, that elements within the US government and covert policy apparatus must have orchestrated or participated in the execution of the attacks for these to have happened in the way that they did} (Emphasis not added). % This doesn't seem related to connection with other conspiracies. 

\paragraph{UFO/Aliens} UFO websites like 9/11 and COVID websites have middling interconnectivity with the other conspiracy theory websites. UFO websites have connections with 16 QAnon websites, 16~9/11 websites,4~COVID websites, and 3~Flat-Earth websites. The major UFO hub is {alienexpanse.com}, a forum site dedicated to the discussion of UFO sightings and alien abductions.



%\todo{Are these authority values important or does it make sense to exclude?}
%\todo{Move category to left most column since that defines what is the top two for each}
%}
%\todo{Might be good to manually verify why this is happening. it's very interesting empirically to show this, but an example would help really solidify what you're showing here.}
%\paragraph{QAnon dominance}

%\todo{Have you considered doing any kind of normalization (e.g., only sampling 99 domains from each set... though that's kind of suspicious) to avoid issues of smaller representation being a reason for smaller intersection?Hans: I have thought about it, but I am worried about picking out 99 sites for each category since obviously which sites I would pick would matter a lot, like a lot. So that is sort of what the HITS analysis is supposed to be for since it gives the amount of interconnections in the entire community and every website has its own shot. Also because I give the amount of domains in each category, people can pretty easily get an idea of what is going on }
%\paragraph{Flat-Earth Weakness}


%\todo{I might cut the ``possible explanation'' part of this unless you have citations, it's hard to justify precisely w/ your data. You might just then merge this into the previous text}
%todo{need a cite on this}
%\paragraph{Other Significant Hubs}
%\todo{What do you want people to takeaway from this section? Try to go one level deeper than just describing the hubs (which is interesting), or even try to work this text into previous sections to provide examples of each conspiracy hub.}
%In addition to the dominant QAnon hubs, various other popular and prominent conspiracy websites play key role key roles within this conspiracy ecosystem. \todo{Maybe an off-path question: If you were to remove 8kun.top from your seed set entirely, would it still play a prominent role? I'm wondering if by seeding w/ 8kun, we're somehow skewing the dataset towards it. Not sure.Hans: Maybe, but 1) we don't see the same phenomena with the other websites that we used to seed, 2) other websites that were not used to seed have similar properties to 8kun.top i.e stillness with 126 connections, 3) 8kun.top is one of the most popular sites so it makes sense why this would be true}
%Several forums in our 97~category agnostic set of websites play prominent roles within the conspiracy ecosystem, though they are not pictured in Figure~\ref{figure:hubs}.
\paragraph{Multiple/Forum Conspiracy Theory Websites} Some of the most connected conspiracy theory websites are uncategorized (``Multiple/Forum''). Most prominently, {8kun.top} is a large repository and gathering place for conspiracy theories. The website where the progenitor of the QAnon conspiracy theory ``Q'' formerly posted ``drops'' or cryptic messages containing secret messages about world events, {8kun.top} points to 98~of the 766~conspiracy theory websites and connects to every category of conspiracy theory (2~Flat-Earth websites, 4~9/11 websites, 7~UFO/Aliens websites, 15~COVID websites, and 70~QAnon websites). Similarly, the now shutdown and former official home for QAnon ``research'' and Reddit clone, {voat.co} had connections to 91~conspiracy theory websites. Finally {stillnessinthestorm.com}, a blog/news site that often posts about QAnon has connections to 126~conspiracy theory sites. Other researchers, including the Columbia Journalism Review\footnote{https://.cjr.org/fake-beta}, have already documented its role in spreading misinformation and conspiracy theories like QAnon. Based on the degree of influence of these types of websites, we see that category agnostic websites and social media websites like {voat.co} play an important part of the conspiracy theory ecosystem, helping to spread and magnify conspiracy theories on the Internet.  

\subsection{Summary}

In this section, we documented the complex and changing role conspiracy theories have had with the wider Internet and in particular the news media. First, we showed that QAnon remains a prominent outlet and repository of conspiracy theories generally, not just those specific to Q. This largely accords with news reporting that QAnon has become a ``big tent conspiracy theory'' that constantly incorporates new claims and theories~\cite{Roose2021}.

Second, we elucidated the commanding role that misinformation plays in interacting with conspiracy theories. As expected, we find that out of the three categories of misinformation, authentic news, and non-news, misinformation websites have by far the most connections with our set of conspiracy theory websites. Websites like {zerohedge.com}, {rt.com}, {breitbart.com}, and {bitchute.com} regularly reference conspiracy theories (and are referenced themselves on these conspiracy theory websites themselves).


We show, chiefly, that the QAnon conspiracy theory is a prominent hub in the conspiracy theory ecosystem and a means by which individuals can connect to other conspiracies. Although QAnon is a relatively new conspiracy theory, it has become a repository and a home for many conspiratorial beliefs ranging from UFO abductions to 9/11 false-flag events. 



\subsection{Determining Granger Causality Directionality}
Utilizing Granger causality, we measure, for instance, if the number of hyperlinks from misinformation websites to conspiracy theory websites is predictive of conspiracy theory websites' popularity. To determine whether a Granger causal relationship is positive or negative, we utilize the cumulative effect of impulse responses. 

Impulse responses measure the response of one time series to the perturbation of the other time series by a single standard deviation (standard deviation is calculated across the entire time series). If the cumulative response from an impulse over time asymptotes to a positive value, we consider the relationship between the two time series as positive and vice versa. This is such that if a sudden standard deviation increase in the number of links from misinformation websites to 9/11 conspiracy theory websites results in an immediate increase in the median popularity of 9/11 websites, but then this increase peters out over time, we count this as a positive relationship. An example of this net cumulative effect is seen in Figure~1%~\ref{figure:nine11-cumulative},
where an increase in hyperlinks results in a cumulative 4000 rank decrease (increase in popularity). Similarly, if the net effect of an increase in the popularity of 9/11 conspiracy theory websites were overall fewer hyperlinks to these sites over time from misinformation websites, we consider this relationship to be negative. If the net cumulative effect asymptotes to zero, we refer to this effect as neutral. We note that determining the \emph{exact} positive and negative effects of changes of a time series on another is a difficult problem that is largely out of scope for this work. 


\begin{figure}
\centering
\begin{minipage}[c]{0.37\textwidth}\label{figure:nine11-cumulative}
\includegraphics[width=\columnwidth]{figures/impulse3.png}
\end{minipage}
\begin{minipage}[c]{0.6\textwidth}
\caption{\textbf{Links from Misinformation Cumulative Impulse Response on Median Popularity of 9/11 Websites}---We show an example of a positive cumulative impulse response. Modelled here is the cumulative increase in popularity (decrease in rank) (with 95\% confidence intervals) in the median popularity of 9/11 websites following a sudden 1 standard deviation increase in hyperlinks from misinformation websites. The cumulative response asymptotes to decrease in rank of 4000 (increase in popularity).}
\end{minipage}
\end{figure}


\subsection{HITS algorithm}
To identify significant websites, we run {Hypertext Induced Topic Selection} ({HITS}) algorithm~\cite{Kleinberg1997} against a domain-centered graph of our websites' connections. 
Per {HITS}, we discern \textit{hub} central and \textit{authority} central domains~\cite{LinkAnalysis}. Hub domains are domains that point to many ``high authority domains and which are themselves high-value domains''. A hub typically has a large out-degree. Authority domains are ``valuable and information-dense domains'' pointed to by many other domains and ordinarily have a high in-degree. 
 %express.co.uk & 2,499,152 \\
 
 \begin{equation}
    X_t = \Sigma^p_{i=1}a_{2i}X_{t-i}
    Y_t = \eta_0 +\Sigma^p_{i=1} \eta_iY_{t-i} + e_t
\end{equation}



To test for Granger causality within this work, we utilize linear vector autoregressive (VAR) models. Two such models are required. The first restricted model assumes that $Y$ linearly depends on the past values of itself and a time-dependent noise term $e$:
%
\begin{equation}
    Y_t = \eta_0 +\Sigma^p_{i=1} \eta_iY_{t-i} + e_t
\end{equation}
where $p$ is the number of past terms of $Y$ that are considered.
The second model assumes that $Y$ depends linearly on the past values of both $X$ and $Y$, and a time-dependent noise term $u$:
%
\begin{equation}
    Y_t = \alpha_0 +\Sigma^p_{i=1}\alpha_iY_{t-i}  +\Sigma^p_{i=1}\beta_iX_{t-i}  +u_t
\end{equation}
where $p$ is the number of past terms of $Y$ and $X$ that are considered.


\begin{table}
\centering
\small
\begin{tabular}{lll}
\toprule
{Category} & {Avg. Harmonic Centrality} & {Avg. Pagerank} \\
\midrule
Multiple/Forum & 1.135 & 0.0241\\ 
QAnon & 0.864 & 0.00118 \\
Flat-Earth &0.477 & 0.00549 \\
COVID & 0.942 & 0.00328 \\
UFO/Aliens & 1.042 & 0.00307\\
9/11 & 1.160& 0.00682\\

\bottomrule
\end{tabular}
\caption{\textbf{Average Harmonic and PageRank centrality measures for each conspiracy theory category}--- Utilizing the full web crawl snapshot of Common Crawl from February 2021 to May 2021~\cite{Nagel2021}, we determine each conspiracy theory website group average harmonic and PageRank centralities. As seen, each group on average is more ``central'' to the web that the average website online by both methods of determining centrality.
}
\label{table:conspiracy-hubs}
\end{table}


\begin{table}
\centering
\small
\begin{tabular}{llllll}
\toprule
{Category} &{QAnon} & {Flat-Earth} & {COVID} & UFO/Aliens & 9/11  \\
\midrule
Misinformation \\
Authentic News \\
Non-News \\
\bottomrule
\end{tabular}
\caption{\textbf{Percentage of Domain to Domain Connections}---The top two most central two websites across the Common Crawled Internet from February 2021 to May 2021~\cite{Nagel2021}, in each conspiracy theory category. The Alexa Rank is given as of March 1, 2021. 
}
\label{table:conspiracy-hubs}
\end{table}


\begin{table}
    \small
    \centering
    \begin{tabularx}{.85\columnwidth}{lrr}
    \toprule
    Conspiracy Theory &  Unique Misinfo Stories  & Unique Authentic News Stories  \\
    \midrule
    QAnon   &   204,995 & 134,213 \\
    COVID   &   3,053,769 & 8,287,353\\
    UFO/Aliens  &   1,603,975 & 1,085,195\\
    9/11 &   1,301,941 & 1,251,490\\
    Flat-Earth&   108,448  & 29,956\\
    \bottomrule
    \end{tabularx}

   \caption{\textbf{Number of Stories Mentioning Each Conspiracy Theory}--- Both Misinformation and Authentic News have written extensively about each conspiracy theory.}
   %\vspace{-15pt}
   \label{table:conspiracy-num-stories-exact}
\end{table}


\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/qanon-connections.drawio.png}
  \caption{QAnon  Connections}
\label{fig:qanon-sub1}
\end{subfigure}%
\begin{subfigure}{.28\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/nine11-connections.drawio (1).png}
  \label{fig:nine11-sub2}
   \caption{9/11  Connections}
\end{subfigure}

\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/covid-connections.drawio.png}
   \caption{COVID  Connections}
   \label{fig:covid-sub2}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/ufo-connections.drawio.png}
   \caption{UFO  Connections}
  \label{fig:ufo-sub2}
\end{subfigure}
\begin{subfigure}{.28\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/flat-connections.drawio2.png}
  \label{fig:flat-sub2}
   \caption{Flat-Earth Connections}
\end{subfigure}

 QAnon \leftarrow & -- & 7.5\%  & 14.9\% &  11.4\% & 12.2\% \\ 
     Flat-Earth \leftarrow & 19.1\% & -- & 11.2\% & 12.6\%& 15.4\%\\
     COVID\leftarrow  &  35.1\% & 10.4\% & -- &  16.6\%& 16.9\% \\
     9/11 \leftarrow  & 21.3\% &9.3\% & 13.2\% &  --- & 14.5\%\\
     UFOs/Aliens \leftarrow  & 15.5\% & 7.6\%  & 9.0\% & 9.7\% & -- \\
     
     
     
 \subsection{Polarization and Conspiracy}
Prior research suggests that polarization can help explain conspiratorial beliefs~\cite{bessi2015science,uscinski2017conditional,bessi2015viral}. For example, researchers have shown that Americans with higher political polarization levels are more likely to believe in birtherism (the conspiracy theory that former President Barack Obama was not born in the United States)~\cite{Enders2018}. In this work, we find that the partisanship levels of news websites have a Pearson correlation of $\rho=0.521$ with a website's shared external domain connections with conspiracy theory websites, increasing to $\rho=0.621$ when only considering conservative-leaning websites. This indicates, reinforcing prior work~\cite{imhoff2022conspiracy} published in Nature, that as societies, websites, and the Internet as a whole become more politically polarized, conspiratorial ideas will increase in tandem. 


\subsection{Tracking Misinformation }
Labeling a website as a peddler of misinformation or as fringe is a difficult thing to do. It requires rigorous fact-checking and objective measures of truth, which are expensive and difficult to obtain. Furthermore, the decision to categorize a website as misinformation or fringe has become intensely political~\cite{LabelingNews}. For example, the site mediabiasfactcsheck.com labels the Washington Post as ``mostly factual'' due to failing two fact checks and using loaded words, despite many considering it a very trusted source~\cite{Watson2021}. 

We argue that given that conspiracy theories are readily identifiable and that the number of shared connections is an objective measure, our metric, which is based on websites' penchants to promote \textit{conspriacy-orietned} materials and their partisanship, can help ameliorate issues surrounding the labeling of websites. When building our presented metric, we note that it is much easier to label large conspiratorial movements than individual news sites that may get some things right and other things wrong. Identifying flat-earth websites is largely uncontroversial. Similarly, for obtaining partisanship scores, Robertson \textit{et al.} used how often Republicans and Democrats linked to given websites on Twitter, another objective measures~\cite{robertson2018auditing}. For those websites not already within their dataset, partisanship levels can be easily obtained using their methodology. As such, using our metric can help introduce a level of objectivity into grading given sites as conspiratorial or as promoting fringe materials. If researchers can use objective metrics, building on previous work in misinformation labeling, they will be able to more effectively identify and further stem the flow of misinformation and fringe material on the Internet.


==> extremism.tex <==
\section{Explaining and Measuring and Misinformation Websites' Fringe and Conspiratorial Attitudes}

In Sections~\ref{sec:ecosystem} and~\ref{sec:temporal}, we explored the interconnectivity between the news media and conspiracy theory ecosystems and showed how misinformation websites promote the growth of conspiracy theories. We now investigate a driving force behind conspiratorial and fringe material online---political polarization. Prior work has suggested that political polarization can help explain conspiratorial beliefs~\cite{bessi2015science,uscinski2017conditional,bessi2015viral}, and according to the Pew Research Center, partisan bias has increased significantly since 1994~\cite{PewPolarization}. Furthermore, this increase in partisanship largely corresponds with the rise in conspiracy theories online (Figure~\ref{figure:time-series-change}). In this section, we thus investigate political polarization's role in the evolution and growth of conspiracy theories.

Specifically, utilizing our lists of conspiracy theory websites and external political polarization data, we show that partisan bias has a $\rho =0.521$ Pearson correlation with websites' graph similarity to conspiracy theory websites. We conclude this section by proposing a new metric to measure websites' fringe attitudes, which objectively measures a website's fringe attitudes by taking into account, partisanship and levels of \textit{conspiracy-oriented} hyperlinking. %and can be utilized to objectively understand a website's orientation to the extreme.

\subsection{Political Partisanship and Similarity to Conspiracy}
\label{sec:polarization-conspiracy}



%\todo{We should chat about if this is the right metric for the task. Seems a bit confusing to follow, not sure what the intention of this metric is (why not just say raw \# of conspiracy sites that a website links to, or as a fraction of their own unique links?)} 
%\todo{This is described already in the methodology, we don't need it in both locations. I'd drop it in one of the two places. Personally, I'd drop the version in the methodology since there's nothing the reader can do with the information at that point in the paper and will probably have forgotten it.}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/polarization_vs_connections.png} 
\caption{\textbf{Partisan bias vs. conspiracy theory similarity}---For news-related domains (i.e, misinformation and authentic news websites), as partisan bias levels increase, websites have a higher percentage of shared domain connections with conspiracy theory websites.}
\label{figure:extremness-v-polarization}
\end{figure}

Although not a causative analysis and limited to US partisanship, we now look to establish whether a website's partisanship level corresponds with its similarity to conspiracy theory websites or its likelihood to post conspiratorial content. For this analysis, we determine whether a website's orientation to conspiracy theories is a function of the website's audience's partisanship, as defined by Robertson \textit{et~al.}'s partisanship bias dataset~\cite{robertson2018auditing}. Robertson \textit{et~al.}'s dataset presents partisanship data on a scale of -1 (liberal/Democratic-leaning) to +1 (conservative/Republican-leaning) for 19K~websites. Cross-referencing this dataset with our curated lists of websites, we find that 192 authentic, 186 misinformation, and 143 non-news websites have scores in Robertson \textit{et~al.}'s dataset~\cite{robertson2018auditing} and that had at least 100 domain connections. For each website in this combined dataset, we define the website’s similarity to conspiracy theory websites as the percentage of external domains that it links to that are \emph{also} linked to by our group of 856 conspiracy theory websites.  This metric is essentially the overlap node similarity metric~\cite{goldberg2010measuring,xie2013overlapping}, giving us an approximation of how similar a given website is to conspiracy theory websites generally. We utilize all domains rather than just \textit{conspiracy-oriented} domains to {fully} capture how the behavior of a website emulates that of conspiracy theory websites. Given our use of connections as a factor, we finally note that filter our dataset to contain only the set of websites having connections to at least 100~other domains, leaving 346 authentic, 156 misinformation, and 143 non-news websites. 

%For each website in this combined dataset, we define a website's similarity to conspiracy theory websites as the the percentage external domains hyperlinked by our list of 856 conspiracy theory websites that this website \textit{also} hyperlinks to.
%are also linked to by our group of 856 conspiracy theory websites.
% The percentages are not necessary as that does not really tell us anything. THe only thing that matters for our study is N, not how much of predefined sets were in another dataset 
%% If it's some tiny small percentage, you could argue that they aren't necessarily representative of the category. Percentage isn't a perfect measure of representivity, but at least gives the reader some sense of whether it says anything. If only something like 3\% of sites are measured, why should I believe the dataset tells me anything about the category? The same could be said across the different conspiracies. If you have other metrics to show representativity, then you could those instead too.

%\todo{It's unclear to me here why you introduce a new metric instead of building on the ones used in the prior section, e.g., connectivity-based ones. Can you provide intuition why it's worth introducing something new?}

%Thus, given a website $x$ and the domains that it links to $X$, and the set of domains linked to by our 863 conspiracy websites $ConspiracyWebsitesDomainLinks$, the conspiracy proximity value is calculated as:
%\begin{align*}
%    Prox \left(x,ConspiracyWebsites) \right) = \frac{| X \cap ConspiracyWebsitesDomainLinks | }{|X|}
%\end{align*}

%\todo{this doesn't sound like it has anything to do with polarization as written, but rather a repeat of what's previously been discussed. Is this new? If so, how is it different? If it's simply a new metric, you might just say that it's new but inline with prior results}
Echoing Section~\ref{sec:ecosystem}, in Figure~\ref{figure:extremness-v-polarization}, we see that individual misinformation websites have the highest average level (55.4\%) of shared domain connections with conspiracy theory websites. Authentic news websites have the second-highest average (34.7\%), marginally higher than non-news websites at (32.2\%). We further observe that for both authentic news and misinformation websites, as partisan bias levels increase, the similarity to conspiratorial websites increases. For authentic news and misinformation, the Pearson correlation values are 0.284 and 0.377 respectively, suggesting a moderate level of correspondence for both groups. For non-news-related sites, partisanship levels have nearly no correlation/slight-correlation with a website's similarity to conspiracy theory websites.

Combining the 156~misinformation and 346~authentic news websites, we observe an overall 0.521~Pearson correlation between political partisanship and similarity to conspiracy theories. We note that for solely conservative/Republican-leaning news websites, this correlation increases to 0.621. For solely liberal/Democratic-leaning news websites, this correlation decreases to 0.284. This indicates that for liberal-leaning news websites, partisanship may not be as prominent a factor in the promotion of conspiratorial material as for conservative-leaning news websites. These results largely agree with concurrent work based on survey data that found across 26 different countries that as polarization increases on both ends of the political spectrum (left and right), conspiratorial thinking increases~\cite{imhoff2022conspiracy}.



\subsection{Measuring Websites' Fringe Attitudes}

US partisanship on the Republican/Democratic spectrum can explain part of how fringe or a website is, but it is not the only factor. Indeed, Robertson \textit{et~al.}~\cite{robertson2018auditing} found that several Russian misinformation websites have little to no US right/left partisan bias. For example, Russian  misinformation websites like {katehon.com} and {globalresearch.ca} do not have a clear place on the US spectrum, and yet both often spread conspiracy theories much more readily than news sites like {cnn.com} and the {dailywire.com} that have liberal and conservative biases. We thus propose to combine these two concepts (political polarization and conspiracy-orientation) to fully understand how websites' fringe attitudes by proposing a new metric that takes into account both of these factors. Given that similarity to \textit{conspiracy-oriented} websites and political polarization levels (as calculated by Robertson \textit{et al.}~\cite{robertson2018auditing}) can be objectively and automatically determined, this new metric can be utilized at scale to identify fringe websites.


For this section, we define \textit{conspiracy-oriented} websites as we did in Section~\ref{sec:over-time} (websites that have more connections to conspiracy theory websites than to non-news or authentic news websites). We use \textit{conspiracy-oriented} websites in this metric to ensure that only connections to more fringe material are considered (the similarity to conspiracy theory metric from Section~\ref{sec:polarization-conspiracy} considers all connections that conspiracy theory websites have, including to benign websites). Given our use of connections as a factor, we again filter this dataset to contain only the set of domains having connections to at least 100~other domains (N=502).

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/svm-20220614.png} 
\caption{\textbf{Utilizing partisan bias and conspiracy orientation to understand websites' ``fringe attitudes''}--- Using a simple threshold on the partisan bias of a website and the number of conspiracy domains that it links to, one can differentiate between authentic news and misinformation. This illustrates the usefulness of these two criteria in understanding websites' fringe attitudes. 
}
\label{figure:classification}
\end{figure}
% todo{classify into what categories? Are you determining what something is extreme? If so, what's correct mean here? Or, are you differentiating between those two categories?} 
%classify into their respective news categories (misinformation vs authentic news) (is that correct? yeah )
%\todo{does it make sense to move this next sentence up a few paragraphs to where you describe the metric?}
Before building our metric, we observe in Figure~\ref{figure:classification} that using simple thresholding on partisanship levels and each website's percentage of \textit{conspiracy-oriented} connections, we can easily differentiate between misinformation and authentic news.
Creating a simple threshold with just these two inputs using an 80\% training subset of our N=502 dataset, we achieve a 97.0\% accuracy on the remaining 20\% test set (using a Support Vector Machine (SVM) to decide on the threshold boundary). Across both all websites considered, this simple thresholoding approach achieved a 93.1\% precision and a false positive rate of 2.6\% in labeling the 20\% test set. Given that misinformation websites generally are more fringe (see Section~\ref{sec:polarization-conspiracy}), this suggests that these two inputs are highly discriminatory in identify fringe attitudes. We again note that both of these inputs can be automatically determined for a given website using their hyperlinks and utilizing Robertson \textit{et al.}~\cite{robertson2018auditing} approach.


Utilizing the drawn boundary for classification, we now define our metric for understanding a website's ``fringe attitudes.'' We define this metric as a function of the distance of each website to the SVM boundary dividing misinformation from authentic news. Namely, we calculate this metric in the same way SVMs calculate class probabilities. SVM probabilities in the binary case are normally calculated utilizing Platt scaling: \begin{math}
P(class|input) = P(y=1|x) = p(x) = \frac{1}{1+exp(-f(x))}
\end{math} where f(x) is a function learned from the training data. For more details on SVMs and Platt scaling see Platt \textit{et~al}.~\cite{platt1999probabilistic}. Thus, in our case, the score for a given website is the probability it is grouped with misinformation websites given its partisanship level and percentage of \textit{conspiracy-oriented} hyperlinks. Derived as such, values vary from 0 (not fringe) to 1 (fringe).

Looking at the scores for the different groups of sites shown in Table~\ref{table:least-coherent}, we see that among the authentic news sites that were misclassified, nearly all were hyper-partisan websites. Thus even among websites that were misclassified as misinformation, most had fringe elements, evidencing our new metric's usefulness. For several, it is questionable whether they are authentic news websites. For example, the most politically extreme and conspiratorial mainstream website, {humanevents.com} is a known far-right hyper-conservative site~\cite{Bittle2021}. On the day of writing (October 1, 2021), the top story on the site is ``THE DUCHESS IS A VICTIM AND FOOTBALL IS GAY'' (emphasis not added).  We further see that the metric was able to correctly identify several misinformation websites that do not fall on US political spectrum. For example, even though globalresearch.ca is not particularly partisan on the US political spectrum, it was still given a high fringe score (Table~\ref{table:least-coherent}).

\begin{table}
    \small
    \centering
    \begin{tabularx}{.49\columnwidth}{Xr}
    \toprule
    Domain &  Fringe Score  \\
    \midrule
    healthnutnews.com    &   ~1.0 \\
    disclose.tv  &   ~1.0 \\
    americanjournalreview.com & ~1.0 \\
    teaparty.org &   ~1.0 \\
    oathkeepers.org        &   ~1.0 \\
    usdefensewatch.com & ~1.0 \\
   thecommonsenseshow.com & ~1.0 \\
    newstarget.com & ~1.0 \\
    guccifer2.wordpress.com& ~1.0 \\
    globalresearch.ca & ~1.0\\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{0.49\columnwidth}{Xr}
    \toprule
    Domain &  Fringe Score  \\
    \midrule
    humanevents.com             &   0.953 \\
    freedomworks.org             &   0.948 \\
    kenyonreview.org       &   0.912 \\
    ronpaulinstitute.org & 0.897\\
    dailywire.com & 0.855 \\
   consortiumnews.com & 0.851 \\
    davidstockmanscontracorner.com               &   0.836\\
    heritage.org             &   0.790 \\
    dissentmagazine.com & 0.719 \\
    amsterdamnews.com & 0.556 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Most  Fringe (\textit{i.e} partisan and conspiratorial) misinformation (left)  and authentic news websites (right)}---Based on the distance of a given website from the boundary dividing misinformation and authentic news, we devise a metric to measure a website's politically extreme and conspiratorial nature. As seen the most fringe mainstream sites are hyper-partisan websites.}
   \vspace{-10pt}
    \label{table:least-coherent}
\end{table}






==> new_data.tex <==

\begin{table}
    \small
    \centering
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
     QAnon &  Unique URLs  \\
    \midrule
    nytimes.com      &   13,106 \\
    thegaurdian.com     &   12,432 \\
    foxnews.com         & 12,194 \\
    washingtonpost.com   &   8,818\\
    cnn.com             & 5,987 \\
    thehill.com   &   5,776 \\
    bloomberg.com &   4,477 \\
    politico.com & 4,215 \\
    washingtonexaminer.com & 4,189 \\
    huffingtonpost.com         &   3,838 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
      COVID &  Unique URLs  \\
    \midrule
    nytimes.com      &   1342 \\
    theguardian.com     &   824 \\
    washingtonpost.com   &   622\\
    cnn.com   &   599 \\
    cnbc.com  &   578 \\
    forbes.com & 508 \\
    nejm.org & 386 \\
    bloomberg.com         &   374 \\
    cbsnews.com       &   335
    \\
    foxnews.com & 327 \\
    \bottomrule
    \end{tabularx}
    
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
      9/11 &  Unique URLs  \\
    \midrule
    nytimes.com      &   2564 \\
    washingtonpost.com     &   2161 \\
    cnn.com   &   1022\\
    cbsnews.com   &   990 \\
    huffingtonpost.com  &   873 \\
    theguardian.com & 824 \\
    msn.com & 783 \\
    yahoo.com         &   768 \\
    examiner.com       &   696
    \\
    usatoday.com & 536 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
      Flat Earth  &  Unique URLs  \\
    \midrule
    nytimes.com      &   534 \\
    washingtonpost.com     &   315 \\
    npr.org   &   219\\
    cnn.com   &   210 \\
    theguardian.com &   186 \\
    eurekalert.org & 173 \\
   wired.com & 172 \\
    newscientist.com         &   122 \\
    theatlantic.com       &   106
    \\
    livescience.com & 92 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
      UFO/Aliens &  Unique URLs  \\
    \midrule
    smithsonianmag.com      &   1541 \\
    universetoday.com     &   1376 \\
    examiner.com   &   1333\\
    livescience.com   &   1153 \\
    popsci.com  &   1026 \\
    theguardian.com & 994 \\
    newscientist.com & 904 \\
    foxnews.com        &   833 \\
    nytimes.com       &   805 \\
   huffingtonpost.com & 735 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Top Authentic News Websites linked to by Conspiracy Groups}---As noted conspiracy websites make high use of news websites, with each group utilizing different authentic news websites to different degrees. All conspiracy groups have The New York Times within their top 10 linked news websites.}
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}







\begin{table}
    \small
    \centering
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    QAnon &  Unique URLs  \\
    \midrule
    zerohedge.com      &   39654 \\
    thegatewaypundit.com     &   20038 \\
    rt.com         & 19418 \\
   naturalnews.com   &   18090\\
    breitbart.com             & 16261 \\
    theepochtimes.com   &   9527 \\
    sputniknews.com &   8597 \\
    bitchute.com & 7681 \\
    beforeitsnews.com & 7604 \\
    nypost.com         &   6911 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Covid  &  Unique URLs  \\
    \midrule
    healthimpactnews.com      &   2909 \\
    bitchute.com     &   804 \\
    naturalnews.com   &   664\\
    zerohedge.com   &   582 \\
    off-guardian.org  &   486 \\
    greenmedinfo.com & 470 \\
    rt.com & 404 \\
    geoengineeringwatch.org        &   357 \\
    breitbart.com       &   311
    \\
    lifesitenews.com & 310 \\
    \bottomrule
    \end{tabularx}
    
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    9/11 &  Unique URLs  \\
    \midrule
    globalresearch.ca      &   2419 \\
    prisonplanet.com    &   2181 \\
    rawstory.com   &   1323\\
    infowars.com   &   1158 \\
    whatreallyhappened.com  &   979 \\
    veteranstoday.com & 912 \\
    informationclearinghouse.info & 891 \\
    wikileaks.org         &   796 \\
    rt.com      &   694\\
    corbettreport.com & 660 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Fla Earth  &  Unique URLs  \\
    \midrule
    breitbart.com      &   63 \\
    bitchute.com     &   57 \\
    naturalnews.com   &   37\\
    rense.com   &   35 \\
    thegatewaypundit.com &   34 \\
    rt.com & 33 \\
  nypost.com & 33 \\
    icr.org         &   30 \\
    zerohedge.com       &   18
    \\
    wnd.com & 16 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    UFO/Aliens &  Unique URLs  \\
    \midrule
    coasttocoastam.com      &   1809 \\
    rt.com     &   509 \\
    sputniknews.com   &   453\\
    collectiveevolution.com   &   437 \\
    disclose.tv  &   401 \\
    abovetopsecret.com & 352 \\
    rense.com & 321 \\
    nypost.com        &   306 \\
    beforeitsnews.com       &   298 \\
   ancient-code.com & 226 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Top Misinformation News Websites linked to by Conspiracy Groups}---As noted conspiracy websites make high use of misinformation websites, with each group utilizing different misinformation news websites to different degrees.}
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}

% Mainstream sites with the most links to each website in each category  
%%


\begin{table}
    \small
    \centering
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    QAnon &  Unique URLs  \\
    \midrule
    huffingtonpost.com     &   472 \\
    theintercept.com         & 134 \\
    commondreams.org             & 62 \\
    theguardian.com   &   58 \\
    alternet.org &   44 \\
    countercurrents.org & 36 \\
   nymag.com & 35 \\
    motherjones.com         &   34 \\
     wired.com         &   30 \\
     slate.com          & 24 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    COVID  &  Unique URLs  \\
    \midrule
    ronpaulinstitute.org     &   30 \\
    motherjones.com     &   18 \\
    foreignpolicyjournal.com   &   14\\
    huffingtonpost.com   &   10 \\
    npr.org &   8 \\
    theguardian.com & 8 \\
    nytimes.com & 6 \\
    politico.com        &   6 \\
    adn.com       &   6
    \\
    marketwatch.com & 4 \\
    \bottomrule
    \end{tabularx}
    
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    9/11 &  Unique URLs  \\
    \midrule
    foreignpolicyjournal.com      &   130 \\
    antiwar.com    &   74 \\
    %dailykos.com   &   56\\
    theintercept.com   &   54 \\
    slate.com  &   18 \\
    countercurrents.org & 14 \\
    commondreams.org & 13 \\
    huffingtonpost.com         &   12 \\
    phillymag.com      &   12\\
    foxnews.com & 8 \\
    nytimes.com & 6 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Flat Earth &  Unique URLs  \\
    \midrule
    theguardian.com      &   26 \\
    techcrunch.com    &   12 \\
   wired.com  &   8\\
    nymag.com   &   8 \\
    foxnews.com &   6 \\
    nj.com & 6 \\
  {der-postillon.com} & 6 \\
    slate.com         &   5 \\
    startribune.com       &   4
    \\
    baltimoresun.com & 4 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    UFO/Aliens &  Unique URLs  \\
    \midrule
    huffingtonpost.com      &   224 \\
    dailykos.com     &   41 \\
    foxnews.com   &   22\\
    americanrifleman.org   &   20 \\
    theguardian.com  &   18 \\
    chron.com & 16 \\
    nytimes.com & 16 \\
    wired.com        &   14 \\
    cnn.com      &   12 \\
   chicagotribune.com & 11 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Authentic News sites with the most links to our list of 863 Conspiracy websites for each conspiracy category} There are exceedingly low rates of connection from authentic news websites to conspiracy websites. The worst offender appears to by the {huffingtonpost.com}.}
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}



\begin{table}
    \small
    \centering
    \begin{tabularx}{.5\columnwidth}{Xr}
    \toprule
    Domain &  Unique URLs  \\
    \midrule
    foxnews.com     &   21746 \\
    huffingtonpost.com         & 21469 \\
    nymag.com             & 15508 \\
    observer.com   &   11977 \\
    alternet.org &   7891 \\
    politico.com & 7538 \\
  theguardian.com & 5619 \\
    humanevents.com         &   4559 \\
     nationalreview.com         &   3725 \\
     nytimes.com          & 3401 \\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Authentic News sites with the most links to Misinformation websites.} }
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}





\begin{table}
    \small
    \centering
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    QAnon &  Unique URLs  \\
    \midrule
    dcclothesline.com     &   7804 \\
    gatesofvienna.net         & 5970 \\
    freedomsphoenix.com             & 2196 \\
    infiniteunknown.net   &   1166 \\
    zerohedge.com &   952 \\
    activistpost.com & 715 \\
  ussanews.com & 565 \\
    pakalertpress.com        &   522 \\
     abeldanger.net         &   510 \\
     darkmoon.me          & 475 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Covid  &  Unique URLs  \\
    \midrule
    healthimpactnews.com     &   2316 \\
    humansarefree.com     &   1102 \\
    freedomsphoenix.com   &   933\\
    naturalnews.com   &   807 \\
    lifesitenews.com &   731 \\
    {collectiveevolution.com} & 642 \\
    ussanews.com & 614 \\
    naturalblaze.com        &   367 \\
    activistpost.com       &   351
    \\
    noqreport.com & 328 \\
    \bottomrule
    \end{tabularx}
    
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    9-11 &  Unique URLs  \\
    \midrule
    freedomsphoenix.com      &   289 \\
    abeldanger.net    &   282 \\
    activistpost.com   &   235\\
    theinternetpost.net   &   136 \\
    zerohedge.com  &   119 \\
    {off-guardian.org} & 114 \\
   antiwar.com & 100 \\
    dcclothesline.com         &   84 \\
    consortiumnews.com      &   76\\
    humansarefree.com       & 52 \\
   % dailykos.com & 60 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    Fla-Earth &  Unique URLs  \\
    \midrule
    thedailysheeple.com     &   8 \\
  pjmedia.com  &   6\\
    dailykos.com   &  6 \\
    freedomsphoenix.com &   4 \\
   counterpunch.org & 4 \\
  publishedreporter.com & 2 \\
    speld.nl         &   2 \\
    dcclothesline.com      &   2
    \\
    darkmoon.me &2 \\
    hotair.com & 2 \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{.3\columnwidth}{Xr}
    \toprule
    UFO/Aliens &  Unique URLs  \\
    \midrule
    coasttocoastam.com      &   332 \\
    abovetopsecret.com     &   98 \\
  
    dailykos.com   &   41 \\
    naturalnews.com  &   36 \\
    {collectiveevolution.com} & 34 \\
   humansarefree.com & 34 \\
    themindunleashed.com        &   18 \\
    theblaze.com      &   18 \\
   pakalertpress.com & 16 \\
   dcclothesline.com & 13 \\
    % dailycaller.com   &   48\\
    \bottomrule
    \end{tabularx}
   \caption{\textbf{Misinformation sites with the most links to Conspiracy websites for each conspiracy category} There are exceedingly low rates of connection from authentic news websites to conspiracy websites. The worst offender appears to by the {huffingtonpost.com}.}
   \vspace{-10pt}
    \label{table:top_link_in}
\end{table}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/alexa_consp_popularity-2013.png} 
\caption{\textbf{Median Alexa Rank of Conspiracy Theory Websites}--- We note. We note a large increase in the median popularity of all conspiracy theories around August 2019. This increase in popularity preceded and was concurrent with both the Christchurch and El Paso mass shootings in New Zealand and the USA. In both cases, the shooters posted their manifestos on the QAnon associated website 8chan.net.   }
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/Minsfomain2fakeOverTime.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/main2fakeOverTime.png} 
\caption{\textbf{Amount of Links to Misinformation Websites}--- Authentic News websites have continually linked to misinformation website. However, following 2012-2013, the sheer amount of links to misinformation websites has decreased. This is despite the fact that the number of misinformation websites has increased throughout the past decade. }
\label{figure:misinfo-main-conspiracy}
\end{figure}

\begin{table}
\centering
\small
\begin{tabular}{lrr}
\toprule
{Misinformation UFO Words} & { Authentic UFO Words} \\
\midrule
new &  credible \\
much-discussed & out-of-this-world \\
sensational &vicious \\
real &top-heavy \\
possible &detailed \\
\bottomrule
\end{tabular}
\caption{\textbf{Links}---The top two domain hubs in each conspiracy category from the network graph built from 848 different conspiracy domains as a root set. Alexa rank from January 1, 2021.}
\vspace{-20pt}
\label{table:conspiracy-hubs}
\end{table}



\begin{table}
\centering
\small
\begin{tabular}{lrr}
\toprule
{Misinformation Flat-Earth Words} & { Authentic News Flat-Earth Words} \\
\midrule
much-maligned &  zetetic \\
falsifiable & skeptic \\
infamous &real \\
newest &idiotic \\
real &false \\
\bottomrule
\end{tabular}
\caption{\textbf{Links}---The top two domain hubs in each conspiracy category from the network graph built from 848 different conspiracy domains as a root set. Alexa rank from January 1, 2021.}
\vspace{-20pt}
\label{table:conspiracy-hubs}
\end{table}




\begin{table}
\centering
\small
\begin{tabular}{lrr}
\toprule
{Misinformation QAnon Words} & { Authentic QAnon Words} \\
\midrule
questionable &  cultish \\
amazing & virtual \\
worthy &moronic \\
untouched &loudest \\
vocal &viral \\
\bottomrule
\end{tabular}
\caption{\textbf{Links}---The top two domain hubs in each conspiracy category from the network graph built from 848 different conspiracy domains as a root set. Alexa rank from January 1, 2021.}
\vspace{-20pt}
\label{table:conspiracy-hubs}
\end{table}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/qanon2.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/covid4.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/ufo4.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/nine114.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/flat-earth4.png} 
\caption{\textbf{Amount of Links to Conspiracy Websites}--- Both Authentic News and Misinformation Websites have linked to  our list of 863 conspiracy domains, with the sheer amount peaking in 2016 for Misinformation websites and in 2013 for Authentic News websites. Following 2016, the amount of links to conspiracy domains from mainstream sites decreased and leveled off, while the amount of misinformation domains dipped before increasing again in 2020.}
\label{figure:misinfo-main-conspiracy}
\end{figure}

==> related.tex <==
\section{Related Work}
\label{sec:related}

While there have not been significant direct studies of the intersection of conspiracy theories and misinformation, there has been considerable prior work about both phenomena.

%The Internet was once hailed as a gateway for everyone in the world to gain unprecedented access to the vast library of human knowledge~\cite{wellman2004three}. However, even as people gain additional access to this library, people have also been exposed to vast quantities of misinformation. Even more so, as social media has exploded and more people have contributed to discussions, false information has spread upwards of 10 times faster than true information~\cite{vosoughi2018spread}. While the absence of gatekeepers has enabled a tremendous growth of different perspectives, it has also caused the emergence of misinformation and ``echo chambers'' that reinforce and confirm biases~\cite{starbird2018ecosystem}. For those stuck in conspiratorial or misinformation ecosystems, this often disallows sometimes lifesaving information from entering their informational bubbles~\cite{mocanu2015collective, roozenbeek2020susceptibility}.
\subsection{Conspiracy Theories}
Despite research literature that indicates that the predilection of people to believe in conspiracy theories has remained somewhat constant across time~\cite{uscinski2014american,van2014power}, various authors have concluded that large spikes in conspiratorial belief often occur following major societal change~\cite{hofstadter2012paranoid,van2017conspiracy}. According to Gallup, at a high point in the early 2000s following September 11, approximately 81\% of the American public believed in at least one conspiracy theory~\cite{swift2013majority}. To understand this phenomenon, Samory \textit{et~al.}~\cite{samory2018conspiracies} used causal time-series analysis to understand changes in conversation and engagement following dramatic world events on the Reddit subcommunity \texttt{r/conspiracy}. They found that after these dramatic events, users on Reddit's \texttt{r/conspiracy} subcommunity show signs of emotional shock as well as increased expressions of both certainty and doubtfulness. Similarly, Bessi \textit{et~al.}~\cite{bessi2015science} found that insular communities and polarized communities often form Facebook groups to discuss and engage with news related to conspiracy theories. 

\subsection{Misinformation Graph Analysis}
Several others have exploited the semantic information that exists in mutual hyperlinking amongst semantically similar domains. As shown in Bhatt \textit{et al.}, Hanley \textit{et al.},  Garimella \textit{et al.}, and Miller \textit{et al.}, semantic information is often embedded within hyperlink graphs ~\cite{bhatt2018illuminating,hanley2021no,garimella2021political,miller2011sentiment}. Bhat \textit{et al.} showed that partisan news producers have a high degree of internal referrals, driving consumers to similar types of websites. Hanley \textit{et al.} showed that QAnon-themed websites often had deeper connections to misinformation compared to authentic news. Garimella \textit{et al.} showed a 0.70~correlation between a given websites' polarization level and the average polarization levels of websites linked to it. Finally, Miller \textit{et al.} showed in their work that the sentiment of posts and blogs often cascades in hyperlink graphs as one post affects another.

Starbird \textit{et~al.}\ and Sehgal \textit{et~al.}\ have further shown that mutual hyperlinking persists across misinformation spreaders~\cite{starbird2018ecosystem,sehgal2021mutual}. Starbird \textit{et~al.}\ built a domain graph of relatively ignominious misinformation campaigns based on shared hyperlinks. Their approach rests on utilizing the Twitter social graph to draw connections between different domains and campaigns. Sehgal \textit{et~al.}\ show that hyperlinks shared between websites and Twitter users can be utilized to identify coordinated efforts to spread disinformation. Their work buttresses this by building a classifier based on mutual link sharing amongst misinformation spreaders on Twitter.

\subsection{Identifying Misinformation}
Several works have attempted to identify misinformation through microblogging messages~\cite{jain2016towards, qazvinian2011rumor, ghenai2017catching}, network infrastructure~\cite{haninfrastructure}, natural language processing~\cite{serrano2020nlp, oshikawa2020survey, gilda2017notice}, and images~\cite{garimella2020images, zannettou2020characterizing, wang2020understanding}. Zannettou \textit{et~al.}\ and Wang \textit{et~al.}\ studied misinformation through shared images~\cite{zannettou2020characterizing,wang2020understanding}. Abdali \textit{et~al.} identified misinformation websites from screenshots on their articles~\cite{abdali2021identifying}. Qazvinian used the linguistic feature present in misinformation articles to identify false or misleading information~\cite{qazvinian2011rumor}. Finally, Hounsel \textit{et~al.}\ utilized network infrastructure-based features to build a classifier to identify misinformation domains as they appear~\cite{hounsel2020identifying}. As shown in Han \textit{et~al.}, misinformation websites often contain particular and specialized infrastructure to avoid bans and to monetize their efforts~\cite{haninfrastructure}. 

Our work examines and measures the impact of specific social phenomena (prominent conspiracy theories), builds on others' contributions to identify the long-term influence of these types of social contagions. In their papers, Wilson and Starbird \textit{et al.} look at the spread of disinformation campaigns related to the Syrian White Helmets, and Hanley \textit{et al.} look at the spread of QAnon~\cite{wilson2020cross,hanley2021no}. Our work further borrows from the history of network analysis pioneered by Kleinberg \textit{et~al.}~\cite{kleinberg1999web}. Kleinberg \textit{et al.} and Park \textit{et al.} used hyperlink graph features to understand key features of the Internet while this network was still in its infancy~\cite{kleinberg1999web, park2003hyperlink}. 
